Polar alignment of a massive retrograde circumbinary disc around an eccentric binary

A test particle orbit around an eccentric binary has two stationary states in which there is no nodal precession: coplanar and polar. Nodal precession of a misaligned test particle orbit centres on one of these stationary states. A low mass circumbinary disc undergoes the same precession and moves towards one of these states through dissipation within the disc. For a massive particle orbit, the stationary polar alignment occurs at an inclination less than $90^{\circ}$, this is the prograde-polar stationary inclination. A sufficiently high angular momentum particle has an additional higher inclination stationary state, the retrograde-polar stationary inclination. Misaligned particle orbits close to the retrograde-polar stationary inclination are not nested like the orbits close to the other stationary points. We investigate the evolution of a gas disc that begins close to the retrograde-polar stationary inclination. With hydrodynamical disc simulations, we find that the disc moves through the unnested crescent shape precession orbits and eventually moves towards the prograde-polar stationary inclination thus increasing the parameter space over which circumbinary discs move towards polar alignment. If protoplanetary discs form with an isotropic orientation relative to the binary orbit, then polar discs may be more common than coplanar discs around eccentric binaries, even for massive discs. This has implications for the alignment of circumbinary planets.

==> response.tex <==
We thank the referee for the useful comments that have improved the manuscript. We have dealt with all of the points raised and outline our responses below. We hope that the paper will be acceptable for publication now. 




This is an interesting paper on a yet to be explored topic on the dynamics of protoplanetary disks orbiting eccentric binaries, and should be published.  As mentioned in the paper, although the dynamics of disks and planets inclined to the orbital plane of an eccentric inner binary have been explored in-detail, an overlooked portion of parameter space are disks and planets starting off retrograde with respect to the inner binary, which may evolve to a retrograde fixed point (e.g. Martin & Lubow 2019).  This work does N-body and SPH simulations to understand the dynamics of planets and disks about this fixed point.  My comments for the manuscript are all minor, and have mainly to do with re-organization, clarifying a few technical points, and a longer discussion on the implications of this work.

The biggest deficiency in the author’s opinion is a almost complete lack of discussion on the astrophysical relevance of this mechanism in the discussion and/or conclusion section.  We know have a number of tracers of disk mass (i.e. Anderson, Zhang et al. 2022; Anderson, Williams, van der Marel et al. 2022).  Since this mechanism depends sensitively on disk mass, how many disks are expected to evolve to this retrograde polar state?  Also, once the disk dissipates, how many planets should also have this inclination?  In addition, how many disks should have the retrograde inclinations required to evolve into this retrograde fixed point, considering how turbulence in giant molecular clouds is the expected way these disks become misaligned in the first place (e.g. Bate 2018)?  The referee understands none of the SPH calculations where able to stay in this retrograde state, but if the authors feel a bit pessimistic about any planets or disks actually being observed in this orientation, they should state this explicitly and why they feel this way.

RESPONSE: We have added some discussion of these points to the conclusions and also included a new sentence in the abstract. 

Figures: At the moment, the figures are placed in a very counter-intuitive order.  Although Section 2 discusses the N-body dynamics, while section 3 discusses the SPH simulations, results from these two sections are placed on the same figures (Figures 1, 2, and 4).  If the N-body and SPH Figures are separated, the referee thinks this would increase the clarity of the manuscript.

RESPONSE: We prefer to keep the figures together for ease of direct comparison between the n-body simulations and the disc simulations. However, we have tried to make the captions clearer which section each figure is described in. 


Also, Figure 2 does a nice job explaining the dynamics of the circulating and librating states, but in the referee’s opinion, should be placed much sooner in the paper (e.g. in the introduction when these different dynamical states are first being discussed).  The figure would look much better if the resolution of the cartoon were increased as well.

RESPONSE: We have increased the resolution of the cartoon figure. We found it difficult to try to incorporate the figure into the introduction since it requires describing the simulation. We prefer to keep the figure where it is but we added a reference to it in the introduction. 

For the SPH simulations, the author does a nice job explaining how the inclination and longitude of the ascending node are calculated for a disk, but neglects how j is calculated.  The author is guessing this is calculated by integrating the initial surface density profile over the radial extent of the disk, and comparing this to the binary angular momentum, but it would be nice if this were stated explicitly.


RESPONSE: We have added some new equations in Sections 2.1 and 3.1 to explain our calculations of the angular momentum ratio.
